Stochastic Prediction of Multi-Agent Interactions from Partial Observations

We present a method that learns to integrate temporal information, from a learned dynamics model, with ambiguous visual information, from a learned vision model, in the context of interacting agents. Our method is based on a graph-structured variational recurrent neural network (Graph-VRNN), which is trained end-to-end to infer the current state of the (partially observed) world, as well as to forecast future states. We show that our method outperforms various baselines on two sports datasets, one based on real basketball trajectories, and one generated by a soccer game engine.

==> text/formulation.tex <==
\section{Formulation}
\label{sec:formulation}

This section describes our problem formulation and the baseline model to tackle the problem.

\subsection{Problem Definition}

Given a sequence of RGB images from video clips, our goal is to identify all the agents in the video, estimate the current state of each individual agent based on visual observation, and predict the future states that are not observed yet. Note that there is no requirement for the ordering of estimation and prediction tasks, they can be interweaved with each other. Take sports videos as an example, the identities could be player names or shirt numbers, the states could be the current locations of the players, and we want to estimate where the players are right now, and where they will go to in the near future.

More formally, we are given a sequence of visual, state pairs $\{(V_1, S_1), (V_2, S_2), ..., (V_T, S_T)\}$ during training time, where $V_i$ is a short video clip that consists of several frames, and $S_j = \{s_1^j, s_2^j, ..., s_O^j\}$ contains the individual states for all agents. During test time, we are given a sequence of previous unseen observations $\{V_1, V_2, ..., V_{\hat{T}}\}$, the goal is to estimate the states $S_t$ for $t\in \{1, ..., \hat{T}\}$ and predict $S_t$ for $t > \hat{T}$.


\subsection{Variational Recurrent Neural Networks}

A variational recurrent neural network (VRNN)~\citep{VRNN} is a special type of variational autoencoder (VAE)~\citep{Kingma2014Auto}, where the VAE is conditioned on the latent state of an RNN. More specifically, let $\mathbf{s}_t$ be the underlying state of some agent $i$ at time $t$, $\mathbf{v}_t$ be the visual observations at time $t$ and $\mathbf{h}_t$ be the hidden states of the backbone RNN at time $t$. Both the prior and posterior distributions of the latent random variable $\mathbf{z}_t$ are Gaussian distributions $\mathcal{N}(\mathbf{\mu}_t^{\text{prior}}, \text{diag}(\mathbf{\sigma}_t^{\text{prior}}))$ and $\mathcal{N}(\mathbf{\mu}_t^{\text{enc}}, \text{diag}(\mathbf{\sigma}_t^{\text{enc}}))$ respectively, the means and standard deviations are computed by
\begin{equation}
\mathbf{\mu}_t^{\text{prior}}, \mathbf{\sigma}_t^{\text{prior}} = \varphi^\text{prior}(\mathbf{h}_{t-1})
\end{equation}
\begin{equation}
\mathbf{\mu}_t^{\text{enc}}, \mathbf{\sigma}_t^{\text{enc}} = \varphi^\text{enc}(\mathbf{h}_{t-1}, \mathbf{s}_t)
\end{equation}
Here $\mathbf{s}_t$ is the ground truth state to be encoded by variational encoder $\varphi^\text{enc}(\cdot)$. Unlike a standard VAE, the prior and posterier are conditioned on the hidden state $\mathbf{h}_{t-1}$ from the RNN backbone, where $\varphi^\text{enc}(\cdot)$ and $\varphi^\text{prior}(\cdot)$ are implemented with neural networks.

We modify the decoder of VRNN to consider visual inputs $\mathbf{v}_t$:
\begin{equation}
\label{eq:vanilla_decoder}
\hat{\mathbf{s}}_t \sim \text{softmax}(\varphi^\text{dec}(\mathbf{h}_{t-1}, \mathbf{z}_t, \mathbf{v}_t))
\end{equation}
Here we use $\text{softmax}(\cdot)$ which discretizes the space of possible states from which $\hat{\mathbf{s}}_t$ is sampled; it can be replaced by other distributions, such as Gaussian. When no visual observation is available, $\mathbf{v}_t$ is set to all zeros. $\varphi^\text{dec}(\cdot)$ is again implemented with neural networks.

The hidden state $\mathbf{h}$ is updated as
\begin{equation}
\mathbf{h}_t = \text{RNN}(\varphi^\text{RNN}(\mathbf{\hat{s}}_t, \mathbf{z}_t, \mathbf{h}_{t-1}))
\end{equation}
where $\text{RNN}(\cdot)$ is the standard recurrent update function, and $\varphi^\text{RNN}(\cdot)$ prepares the inputs to RNN. Here we set $\varphi^\text{RNN}(\cdot)$ as a simple concentenation operation.

\textbf{Training:} The model is trained to perform both estimation and prediction tasks, by maximizing $\sum_{i=1}^N\log P(S_1^{(i)}, ..., S_T^{(i)}, ..., S_{T+\Delta T}^{(i)} | V_1^{(i)}, ..., V_T^{(i)})$ over all $N$ training examples. The probability $P$ is a marginal distribution over $\mathbf{z}$. For each example $i$, we maximizes its lower-bound:
\begin{equation}
\sum_{t=1}^{T+\Delta T}(-\text{KL}(\mathcal{N}(\mathbf{\mu}_t^{\text{enc}}, \text{diag}(\mathbf{\sigma}_t^{\text{enc}})) \parallel \mathcal{N}(\mathbf{\mu}_t^{\text{prior}}, \text{diag}(\mathbf{\sigma}_t^{\text{prior}}))) + \log P(\mathbf{s}_t | \mathbf{z}_{\leq t}, \mathbf{v}_{\leq t}, \mathbf{s}_{\le t}))
\end{equation}

\cs{In implementation section, mention that each time step is weighted differently, weight is $\text{max}(\frac{t}{T}, 1)$. Also mention that we use scheduled sampling, and KL annealing.}

\textbf{Discussion:} Unlike a sequence-to-sequence model, where the RNN backbone consumes visual inputs $\mathbf{v}$ to update its internal states, we decouple the model into a dynamics model for underlying states, where the future is uncertain; and a visual detector from visual inputs, whose goal is to reduce the uncertainty. The only place where they interact is via $\mathbf{\hat{s}}_t$. When we set $\varphi^\text{dec}(\mathbf{h}_{t-1}, \mathbf{z}_t, \mathbf{v}_t) = \varphi^\text{dec}(\mathbf{h}_{t-1}, \mathbf{z}_t)$, the model becomes a standard VRNN. After all, we are interested in estimating and predicting the underlying states that explain the visual observations. The latent noise $\mathbf{z}$ is supposed to explain the multiple plausible futures of the states, and the visual observations are irrelevant here.

However, in the above model, a key missing component is the notion of uncertainty. When $t=0$, the dynamics model is useless and the state estimations could only come from visual inputs. Similarly, when an agent is occluded or out of field of view, the dynamics model could be much more informative than visual inputs. Ideally, we'd like to know how certain each module is, and who should be trusted.
